YASMIN: a Real-time Middleware for COTS Heterogeneous Platforms

Commercial-Off-The-Shelf heterogeneous platforms provide immense computational power, but are difficult to program and to correctly use when real-time requirements come into play: A sound configuration of the operating system scheduler is needed, and a suitable mapping of tasks to computing units must be determined. Flawed designs may lead a sub-optimal system configurations and thus to wasted resources, or even to deadline misses and failures. We propose YASMIN, a middleware to schedule end-user applications with real-time requirements in user space and on behalf of the operating system. YASMIN provides an easy-to-use programming interface and portability. It treats heterogeneity on COTS heterogeneous embedded platforms as a first-class citizen: It supports multiple functionally equivalent task implementations with distinct extra-functional behaviour. This enables the system designer to quickly explore different scheduling policies and task-to-core mappings, and thus, to improve overall system performance. In this paper, we present the design and implementation of YASMIN and provide an analysis of the scheduling overhead on an Odroid-XU4 platform. Last but not least, we demonstrate the merits of YASMIN on an industrial use-case involving a Search & Rescue drone.

==> sections/oldimplementation.tex <==
\section{\label{sec:implem}\LibName~ Design \& Implementation}

We first present the overall architectural concept, before presenting the details of the major scheduling classes. \LibName~ is highly modular and allows (1) the use of various scheduling policies and (2) easy switching between them at compile time throughout macros definitions. 


\ignore{
\LibName~ is exclusively executed in OS user-space, which allows us to use an unmodified OS kernel. Kernel modifications are cumbersome, difficult and error-prone. But, user-space execution requires an initial step to configure the OS in order to 
% remove as much as possible the
minimise the effects of
interferences generated by other system tasks. These configurations are common and have been described several times already \cite{mollison2013bringing, hartig1998taming, saranya2014implementation, brosky2003shielded, rouxel2020prego}.
}

We designed \LibName~ as a library to be compiled individually and linked to the end-user program. We implemented \LibName~ following real-time coding guidelines to enable the use of WCET analysis tools, such as AbsInt's aiT \cite{ferdinand2004ait} or Heptane \cite{hardy2017heptane}, i.e.~we refrain from dynamic memory allocation and loops are statically bounded. To accomplish this, we make use of C-header configuration to define constants used throughout the library, e.g.~the number of threads and the number of tasks. Moreover, we verified our code using PC Lint Plus \cite{pclint} against MISRA-C 2012 rules.

\LibName{} is compatible with any POSIX compliant OS. However, we also rely on the non-POSIX \textit{pthread\_set\_affinity\_np} function that binds a thread to a specific core. Similar requirements can be found in previous works \cite{mollison2013bringing, saranya2014implementation}.

\subsection{\label{ssec:implem:gen}Overall Architecture}

We rely on the concept of shielded processor, as described in \cite{saranya2014implementation,brosky2003shielded}. The idea is to reserve cores to only execute real-time tasks in order to minimise interference with system tasks. On each of the reserved cores a thread is spawned, hereafter called a worker thread, which is then responsible for executing the Real-Time (RT) tasks. The worker thread serves as a container for the execution of the user RT tasks, which sees it as a virtual CPU.

The library is configured at compile time using a configuration file. In this file, pre-processor definitions set, among others, the type of scheduling, the type of mapping and the priority assignment. The configuration is applied for the whole compiled binary, only one scheduling policy is allowed at a time, therefore to switch to another one, the whole application needs to be recompiled with new parameters.% These setup parameters are mutually exclusive, which means it is not possible to have some threads with an off-line scheduling policy while others would be using an on-line one.

%\begin{table}[ht]
%    \centering
%	\caption{General API of \LibName}
%	\label{tbl:implem:api}
%	\begin{tabular}{|l|l|}
%		\hline
%		void \APIprefix init(void) & Initialise the coordination runtime library\\
%		\hline
%        void \APIprefix start(void) & Start to execute the tasks of the application\\
%		\hline
%		void \APIprefix stop(void) & Stop the application\\
%		\hline
%		void \APIprefix cleanup(void) & \makecell[l]{Wait for all threads to finish and close}\\
%		\hline
%		\end{tabular}
%\end{table}

\input{sections/API}

% \begin{lstlisting}[language=C,caption=General C code example,label=fig:implem:glob:snippet]
% void main(int argc, char **argv) {
%     @\APIprefix@init();
%     // add tasks
%     @\APIprefix@start();
%     //schedule is running, wait for some event
%     @\APIprefix@stop();
%     @\APIprefix@cleanup();
% }
%     \end{lstlisting}

Table~\ref{tbl:implem:api} presents the general API of \LibName. All functions are prefixed with \APIprefixName, which we leave out in the paper for conciseness. The end-user program must first call the \textit{\APIprefix init} function that initialises different structures of our library. Then, the user must declare the various tasks using the API described in the following sections. 

At this stage, no user code has yet been executed, and no scheduling has been performed. It is after the call to \textit{\APIprefix start} that the scheduler starts to run the application. Calling the \textit{\APIprefix stop} function stops the scheduler. Then, either the main program performs the finalisation of the application with \textit{\APIprefix cleanup}, or the schedule can be resumed with a new call to \textit{\APIprefix start}. It is possible to alter the taskset only when the schedule is not running, hence enabling multi-mode scheduling\cite{goossens2019acceptor}. The function to alter the taskset are skipped from the following APIs tables, due to space constraints.
%It is not possible to add, remove or alter tasks while the schedule is being executed (i.e.~between two successive calls to \textit{\APIprefix start} and \textit{\APIprefix stop}). However, as soon as the scheduler is paused/stopped, the main program can alter the task set, modify timing parameters and so on.

%Calls to the end-user RT tasks are surrounded by hooks. The \textit{pre-hook} is called before calling a task, and the \textit{post-hook} is called after the completion of a task. These hooks are optional and configured at compile time. They enable a powerful and modular mechanism to alter the scheduling. For example, the pre-hook function can switch between versions of tasks depending on the current system status, e.g.~the battery load status.
%A post-hook function could, among others, be used to detect deadline misses. These pre/post-hook functions are user-provided and their overhead is properly accounted for.

\begin{figure}[ht]
    \begin{subfigure}{0.33\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Off-Line-Sched.pdf}
    	\caption{On-line dispatcher with an off-line scheduling strategy. 
    	Each worker thread is pinned to a core, and a scheduling loop iterates on its ready task queue.}
    	\label{fig:implem:off-line}
	\end{subfigure}
	\begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Part-On-Line-Sched.pdf}
    	\caption{Partitioned on-line scheduling strategy. 
    	A scheduler thread pinned to another core feeds each worker thread ready task queue.}
    	\label{fig:implem:part-on-line}
    \end{subfigure}
    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Glob-On-Line-Sched.pdf}
    	\caption{Global on-line scheduling strategy. 
    	The ready task queue is now shared among worker thread.}
    	\label{fig:implem:glob-on-line}
    \end{subfigure}
    \caption{Overall architecture for each scheduling class.}
    \label{fig:implem:overview}
\end{figure}

Each different scheduling strategy requires different mandatory information to perform adequately. The code of the different functions of the API is adapted following the defined macros in the configuration file. For example, it is mandatory to provide the release offset of tasks for an off-line scheduling strategy, while it is not for on-line scheduling. 

\subsection{\label{ssec:implem:off-line}Off-line Scheduling}

An \textit{off-line} schedule is computed before executing the application using the timing properties of the task graph set. 
In our run-time implementation an \textit{on-line} dispatcher dispatches tasks at the predefined time following a given time table, a given mapping, and preselected versions.

Figure~\ref{fig:implem:off-line} presents the overall architecture for the off-line scheduling strategy. Each worker thread is pinned to a specific core and has access to a predefined sequence of RT tasks ordered by increasing release time. Upon creation each worker thread starts executing an infinite loop running the RT task in order. To respect the release time of each task (computed off-line), special delay slots are added in between RT tasks, and make the worker thread waits for a pre-computed duration. Delay slots implementation may vary according to the given configuration: 
\begin{enumerate*}
\item \textit{sleep} (default): calls some kernel code, which is hardly timing-analysable, 
\item \textit{spinlock}: enable a more precise overhead analysis at the cost of potential energy waste.
\end{enumerate*}

%\begin{table}[ht]
%    \centering
%	\captionof{table}{\label{tbl:implem:off-line}On-line dispatcher API for off-line schedulers}
%	\scriptsize
%	\begin{tabular}{|l|l|}
%		\hline
%		\makecell[l]{TaskID \APIprefix task\_decl(\\
%		\quad u64 release\_offset, \\
%		\quad u16 virt\_core\_id)} & \makecell[l]{Append a statically scheduled \\task with its release offset \\and mapping\\
%        typedef void (*FuncPtr) (void*)}\\
%		\hline
%		\makecell[l]{void \APIprefix alter\_offset(\\
%		\quad CoordTaskID, u64 new\_offset)} & \makecell[l]{Alter the release offset of a task}\\
%		\hline
%		\makecell[l]{void \APIprefix alter\_mapping(\\
%		\quad CoordTaskID, u16 new\_mapping)} & Alter the mapping of a task\\
%		\hline
%		void \APIprefix rm(CoordTaskID) & \makecell[l]{Remove a task from \\the static schedule}\\
%		\hline
%	\end{tabular}
%\end{table}

% \begin{figure}[ht]
    % \centering
    \begin{lstlisting}[language=C,caption=C code example using the On-line dispatcher API, label=fig:implem:off-line:snippet]
#define S2NS(X) X*1000000000 // convert sec to nsec
void taskA(void *arg) { /*do something*/ }
void main(int argc, char **argv) {
    TaskID aid; TaskData a;
    @\APIprefix@init();
    @\APIprefix@task_init(&a);
    a.release_offset = S2NS(1);
    a.virt_core_id = 0;
    aid = @\APIprefix@task_decl(&a);
    @\APIprefix@start();
    // schedule is running, wait for some event
    @\APIprefix@stop();
    @\APIprefix@cleanup();
}
    \end{lstlisting}
    % \caption{C code example using the Off-line scheduling API}
    % \label{fig:implem:off-line:snippet}
% \end{figure}

Table \ref{tbl:implem:off-line} displays the API to register statically scheduled RT tasks; Figure~\ref{fig:implem:off-line:snippet} shows a code snippet illustrating the use of the API. The \textit{\APIprefix task\_decl} function adds a task in the dispatcher task list providing a function pointer to the task's code, %a pointer to an argument to the task, 
a release time offset relative to the beginning of the schedule and the virtual core/thread id to map the task on.

\textbf{Limitations: }
We do not support preemption in off-line generated schedules. This limitation could easily be overcome by splitting the to be preempted task into two separate subtasks. 
We consider heterogeneous resource management%, e.g. a specific accelerator device as a GPU, 
to be handled by the off-line scheduling step. A task can therefore pilot an accelerator without requesting access to the on-line dispatcher.

\subsection{\label{ssec:implem:part-on-line}Partitioned \& Global On-line Scheduling}

As opposed to an on-line dispatcher for off-line schedules, an on-line scheduler must activate tasks following their arrival time (period), decide which version of the task to execute, and dispatch tasks to a worker thread (or virtual CPU). Two modes are available, \textit{Global} when all tasks can be executed on any virtual CPU, \textit{Partitioned} when all tasks have a predefined target virtual CPU.

Figures \ref{fig:implem:part-on-line} and \ref{fig:implem:glob-on-line} present the overall architecture for, respectively, a partitioned and a global scheduling strategy. In both cases, each worker thread is pinned to a specific core, and have access to a ready queue. The ready queue is filled by a scheduler thread also pinned to its private core, hence minimising interference with worker threads and system tasks. Difference between partitioned and global scheduler implementation lies in the ready queue, where each worker thread has its own ready queue while a single shared ready queue is shared for global scheduling. Final compiled implementation is decided through the configuration given by the user through macros definitions. Only one of the two options is available at a time, hence only one option is finally compiled in the resulting binary.

In both cases, global and partitioned, the ready queue is filled by a extra scheduler thread also pinned to its private core. Unlike \cite{saranya2014implementation}, which also uses a external scheduler thread, our scheduler thread do not constantly check for new tasks to activate. Instead, we periodically checks for new tasks to schedule. It means, that between two activations, the scheduler thread either sleeps or spinlocks, depending on the user configuration, similar to the delay tasks in off-line scheduling discussed in Section~\ref{ssec:implem:off-line}. The period of the scheduler thread is determined using the Greatest Common Divisor (GCD) of all the declared task periods.

Using a separate scheduler thread that executes on its own core decreases the possible parallelism of the application. Indeed, one few core is available to execute user RT tasks. However, you gain in predictability. For example, the way task preemption is realised by the Linux scheduler is to have a periodic interrupt handler that stops the current executing thread, on each core. This interrupt handler, from the kernel, checks if there is a higher priority task to execute. This interruption mechanism must be accounted in the Worst-Case Response Time (WCRT) of user real-time tasks. However in practice, it is very difficult to estimate the time spent in this interrupt handler, introducing pessimism in the WCRT of taks. By using a separate scheduler thread to check for higher priority tasks prevent this practical pessimism, see Section \ref{ssec:implem:other} for details on how we deal with preemption. 

In addition, it is possible to configure the Linux kernel to prevent aforementioned periodic user thread interrupts: a value of $-1$ needs to be written in the virtual file XXX . We refer, the interested reader on how to increase user control over time in Linux, to \cite{rouxel2020prego}.




%Figure \ref{fig:implem:part-on-line} presents the overall architecture for a partitioned on-line scheduling strategy. Each worker thread is also pinned to a specific core, and have access to a ready queue. The ready queue is filled by a scheduler thread also pinned to its private core, hence minimising interference with worker threads and system tasks. 


\LibName~ supports static and dynamic priority assignments following task periods (rate monotonic), deadlines (deadline monotonic, earliest deadline first) or any statically user-defined priorities.
Once RT tasks have been added to their assigned ready queue, and if dynamic priority assignment is employed, then the scheduler must compute the priorities of all tasks present in each ready queue. 
%This step is not necessary for static priority assignment, as tasks priority do not change over time. 
Then each ready queue is reordered by decreasing priority, i.e.~the task with the highest priority always is at the head of the ready queue.
%
After reordering a ready list, a POSIX signal is sent to the thread executing a RT task with a lower priority than that of the new head of its ready queue. Upon reception of the signal, an interrupt handler set up in the thread stops the current task, fetches the new higher priority RT task and switches the execution context. 
%This preemption signal+switching overhead is accounted for in Section \ref{sec:overhead}.

\LibName~ supports recurring and non-recurring tasks. Both type of tasks must be declared before use, but only recurring task make period to be a mandatory information to set in the TaskData structure. Then it is possible for a user-function to activate a non-recurring task whenever it pleases it. The task is then put into the ready queue with a lower priority than recurring task.

\LibName{} supports graph-based tasks. We provide a mechanism to declare and manage FIFO channels required between causally dependent tasks within a graph. The pre-processor macro \textit{\APIprefix channel\_decl} defines the FIFO channel buffer. The channel is then accessed by user task with \textit{channel\_push} and \textit{channel\_pop} functions to respectively push a data and pop a data from the channel. With graph-based task, only the root nodes need to have a period attached, the following nodes are automatically activated by the scheduler ones all required incoming data are present in its connected input channels. 
%Under the hood, the implementation of the \textit{\APIprefix push\_NAME} verifies if there is enough tokens to activate the succeeding task, therefore releasing the need for synchronisation.

\textbf{Limitations:} 


%\begin{table}[ht]
%    \centering
%	\caption{\label{tbl:implem:part-on-line}API available to use an on-line scheduling strategy}
%	\scriptsize
%	\begin{tabular}{|l|l|}
%		\hline
%		\makecell[l]{CoordTaskID \APIprefix decl\_task\_X(\\
%		\quad FuncPtr f,\\
%		\quad void *ud,\\
%		\quad void *var\_properties,
%		\quad Y)
%		} & \makecell[l]{Declare a task with no activation pattern\\
%		\quad$X=priority (P)\rightarrow Y=u32~p$\\
%		\quad$X=deadline (D)\rightarrow Y=u64~d$\\
%		\quad$X=mapping (M)\rightarrow Y=u16~m$}\\
%		\hline
%		\makecell[l]{CoordTaskID \APIprefix decl\_rec\_task\_X(\\
%		\quad FuncPtr f,\\
%		\quad void *ud,\\
%		\quad u64 period,\\
%		\quad Y)
%		} & \makecell[l]{Append a periodic task with different \\requirements $X \in \{P,D,M\}$}\\
%		\hline
%		\makecell[l]{void \APIprefix activate\_task(\\
%		\quad CoordTaskID i)} & \makecell[l]{Activate a task for immediate schedule with}\\
%		\hline
%		\makecell[l]{void \APIprefix alter\_X(\\
%		\quad CoordTaskID i,\\
%		\quad Y)} & \makecell[l]{Alter a property of a task\\ $X \in \{T,P,D,M\}$}\\
%		\hline
%		void \APIprefix rm(CoordTaskID) & Remove a periodic task\\
%		\hline
%		\makecell[l]{CoordVersID \APIprefix add\_version(\\
%		\quad CoordTaskID,\\
%		\quad FuncPtr f,\\
%		void *var\_properties)} & \makecell[l]{Add a version to the task \\with user specific properties}\\
%		\hline
%		\makecell[l]{void \APIprefix use\_version(\\
%		\quad CoordTaskID t,\\
%		\quad CoordVersID v)} & \makecell[l]{User version $v$ for \\next invocation (job) of task $t$}\\
%		\hline
%	\end{tabular}
%\end{table}

% \begin{figure}
    % \centering
%    \begin{lstlisting}[language=C,caption=C code example using the partitioned on-line scheduling API with user-defined priority,label=fig:implem:on-line:snippet]
%@\APIprefix@decl_channel(RecurTask, NextTask, int, 1, r2n);
%void RecurTask(void *arg) {
%    int a;
%    //do something with a
%    @\APIprefix@push_r2n(a);
%    @\APIprefix@notify_r2n();
%}
%void NextTask(void *arg) {
%    int b;
%    @\APIprefix@pop_r2n(&b);
%    // do something with b
%}
%typedef struct {uint32_t param;} taskAparam;
%void TaskA(void *arg) {
%    taskAparam *tAp = (taskAparam*)arg;
%    //do something else
%}
%void pre_hook(CoordTaskData *task) {
%    //if GPU is free and task has a gpu version
%    // then use the gpu version for the current job to execute
%}
%void main(int argc, char **argv) {
%    CoordTaskID r, n;
%    taskAparam tAp;
%    @\APIprefix@init();
%    r = @\APIprefix@push_task_T_P_M(RecurTask, NULL, S2NS(1), 1, 0);
%    n = @\APIprefix@decl_task(nexTask, NULL, 1, 0);
%    @\APIprefix@connect_channel(r, n, r2n);
%    @\APIprefix@start();
%    tAp.param = ...;
%    //wait for some event
%    @\APIprefix@push_task_P_M(TaskA, &tAp, 3, 0);
%    ...
%}  
%    \end{lstlisting}
    % \caption{C code example using the partitioned on-line scheduling API}
    % \label{fig:implem:on-line:snippet}
% \end{figure}

%Table \ref{tbl:implem:part-on-line} shows the API for our partitioned on-line scheduling strategy and 
%Figure~\ref{fig:implem:on-line:snippet} shows a code snippet to illustrate global on-line scheduling.

%Our on-line scheduler implementation allows to add recurring tasks with the function call \textit{\APIprefix decl\_rec\_task\_X}. Due to the absence of function overloading in C, we define multiple preprocessor macros to allow all possible configurations of recurring tasks.
%that we skipped for clarity and space constraints. 
%As an example, \textit{\APIprefix decl\_rec\_task\_M} takes a period and a mapping for the task, whereas the deadline is implicitly set to the period and the priority assignment is postponed until runtime. 
%As another example, \textit{\APIprefix decl\_rec\_task\_P\_D\_M} sets the period, priority, deadline and mapping for a recurring task.

%Different version can be added for recurring tasks using \textit{\APIprefix add\_version}. Then the populated list of versions can be accessed from a pre-hook function (as shown in Listing~\ref{fig:implem:on-line:snippet}). 
%The user-defined pre-hook accesses user-defined properties for a version (e.g.~a structure with resource accesses or energy consumption) and can modify the version to use for the next task invocation with \textit{\APIprefix use\_version}.

%In addition to recurring tasks, arbitrary activated RT tasks can be declared using \textit{\APIprefix decl\_task\_X} (note the absence of the $rec$ mark, and the identical possibility to set different properties). These tasks can be activated at any point in time using \textit{\APIprefix activate\_task}. They are placed in the ready queue at the next invocation of the scheduler. Like recurring tasks their priority depends on the configured priority assignment algorithm. 

\textbf{Limitations: } 
Arbitrary tasks are not yet handled in a conventional way using a recurring server. This is left for future work. On the other hand, this mechanism allows us to further support graph-based task model, see Section \ref{ssec:implem:graph}.

%\subsection{Global On-line Scheduling}

%Unlike the partitioned on-line scheduler with off-line mapping, our global on-line scheduler
%also decides on which core to execute which task.
%Switching from partitioned on-line scheduling to global on-line scheduling moves the ready task queue from worker threads to a higher level. 
%Instead of having one ready queue per thread, we now employ a single shared ready queue. 
%Figure~\ref{fig:implem:glob-on-line} illustrates this evolution.

%The API for global on-line scheduling is the same as for partitioned on-line scheduling presented in Section~\ref{ssec:implem:part-on-line}, except that no mapping information needs to be given when declaring a task.
%If nonetheless provided, our library ignores mapping information.
%This design choice is meant to facilitate switching between scheduling policies without much code rewriting. Consequently, the same code snippet still applies, only the configuration file needs to be modified accordingly.

%\paragraph*{Limitations} 
We do not support job migration, a job (task instance) spawned on a virtual CPU cannot be migrated to another one. However, we do support task migration: job $i$ of some task may run on one virtual CPU while job $i+1$ runs on a different virtual CPU.

We only deal with Directed Acyclic Graph (DAG) tasks, other graph-based task models, such as Synchronous DataFlow (SDF) graph \cite{lee1987static}, must be \textit{a priori} transformed (or expanded for SDF) to cope with a DAG task model. We plan to further implement the concept of delay tokens to cope with cycles in graphs.

\subsection{Heterogeneity}

Tasks may wish to access a specific compute unit. For example, a task design for the GPU first starts on a CPU core, then requests access to the GPU, spawns the GPU kernel, and finally comes back to the CPU core. We implemented resource reservation primitives, Table \ref{tbl:implem:hetero}, to notify the scheduler thread that the resource is being occupied by a task. Then, the worker thread that issues the request is stalled waiting for the access to be released, and no preemption can occur. An asynchronous mechanism allowing the worker thread to execute other tasks while the other computing unit is being used is part of our future work.

In case a second task requests access to the same computing unit in the meantime from a different worker thread, and if the second task has a higher priority, then we apply a Priority Inheritance Protocol (PIP) \cite{rajkumar2012synchronization}.
%priority inversion mechanism. 
Whether or not a priority inversion occurs, the second request is stalled waiting for the first one to complete. 

\begin{table}[ht]
	\caption{API available to request resource}
	\label{tbl:implem:hetero}
	\begin{tabular}{|l|l|}
	    \hline
	     \makecell[l]{void \APIprefix decl\_resource(\\
	     CoordRessID name)} & Declare a resource identified by name \\
	    \hline
	     \makecell[l]{void \APIprefix get\_resource(\\
	     CoordRessID name)} & \makecell[l]{Lock or wait for the resource \\identified by name}\\
	     \hline
	     \makecell[l]{void \APIprefix release\_resource(\\
	     CoordRessID name)}& Release the resource identified by name\\
	     \hline
	\end{tabular}
\end{table}

Heterogeneity is not limited to the use of accelerators, but nowadays is also present in CPU types. For example, a ARM big.LITTLE processor features slow, energy efficient cores (LITTLE) and fast, energy greedier cores (big). Applying resource reservation for this type of heterogeneity does not make sense as the same code can be executed on both cores. We handle this scheme the simplest way, each core still executes its own worker thread. For a partitioned strategy (off-line scheduling, or partitioned on-line), an off-line algorithm already decided which task should be executed on which core. On the other hand, with global scheduling, we either take a semi-partitioned approach, or no specific decision is made. In case two different versions of the task are available, each targeting one of the specific core, a pre-hook can select the most appropriate version to meet the timing constraints. 

% If a single version targeting a specific type of core is present, the same rule applies. If the task version is not built for a particular type of core, then the first worker thread accessing the queue takes the task, whether on which physical core type it is pinned to. In this last case, we advocate that the \textit{a priori} performed schedulability analysis should have accounted for all core types.

\textbf{Limitations: }
For future work, we plan to implement a proxy thread mechanism where resource specific task are moved to this thread while using the resource. This will enable us to not stall the worker thread, but execute other RT tasks.

\subsection{\label{ssec:implem:graph}Task Dependencies}

\begin{table}[ht]
	\caption{API available to request resource}
	\label{tbl:implem:dep}
	\begin{tabular}{|l|l|}
	    \hline
	     \makecell[l]{\APIprefix decl\_channel(\\
	     \quad name
	     \quad datatype,\\
	     \quad size)}&  \makecell[l]{Preprocessor macro to declare a \\FIFO channel identified by name for \\
	     a given datatype and with a storage capacity \\
	     of size}\\
	     \hline
	     \makecell[l]{\APIprefix connect\_channel(\\
	     \quad CoordTaskID src,\\
	     \quad CoordTaskID sink,\\
	     \quad name)}&  \makecell[l]{Preprocessor macro to connect src and sink\\ with channel identified by name}\\
	    \hline
	     \makecell[l]{void \APIprefix push\_NAME(\\
	     \quad datatype d)}& \makecell[l]{Push a value of data-type in the FIFO \\identified by NAME}\\
	     \hline
	     \makecell[l]{void \APIprefix notify\_NAME(\\
	     \quad datatype d)}& \makecell[l]{Notify the scheduler that the source pushed \\
	     all required data in the FIFO identified by \\NAME}\\
	    \hline
	     \makecell[l]{void \APIprefix pop\_NAME(\\
	     \quad datatype *d)}& \makecell[l]{Pop a value of data-type in the FIFO \\identified by NAME}\\
	    \hline
	\end{tabular}
\end{table}

We provide a mechanism to declare and manage FIFO channels required between causally dependent tasks within a graph. Table~\ref{tbl:implem:dep} displays the API elements, and their used in C-code snippet in Listing~\ref{fig:implem:on-line:snippet}. The pre-processor macro \textit{\APIprefix decl\_channel} defines the FIFO channel buffer and the related \textit{\APIprefix push\_NAME}, \textit{\APIprefix notify\_NAME}, and \textit{\APIprefix pop\_NAME} primitives which can then be used by tasks. 
%Under the hood, the implementation of the \textit{\APIprefix push\_NAME} verifies if there is enough tokens to activate the succeeding task, therefore releasing the need for synchronisation.

\textbf{Limitations:} 
We only deal with Directed Acyclic Graph (DAG) tasks, other graph-based task models, such as Synchronous DataFlow (SDF) graph \cite{lee1987static}, must be \textit{a priori} transformed (or expanded for SDF) to cope with a DAG task model. We plan to further implement the concept of delay tokens to cope with cycles in graphs.

\subsection{Further Implementation Aspects}

This section describes other design issues we encountered and how we addressed them in \LibName.

\textbf{Compilation: }
In case of tasks with multiple versions with on-line scheduling, the scheduler is responsible for selecting the proper task version to execute. Therefore, all task versions must be present in the compiled binary executable. This assumption can result in large binary files. To lower its size, the end-user can decide to \textit{a priori} select task versions likely to be used.

\textbf{Accessing time: }
We access time using the POSIX primitive \textit{clock\_gettime} where the given clock can be set using the configuration file. As default, \textit{CLOCK\_MONOTONIC} is employed. It gives a monotonic increasing clock with nanoseconds precision. The POSIX standard does not specify what the time $0$ means, in Linux implementation it corresponds to the earliest system boot time. In our library, we store the time at which the schedule is started, using API call \textit{\APIprefix start} Section \ref{ssec:implem:gen}, then all timing information are computed using this initial starting time.

\textbf{Pre-emption: }
\LibName~ supports pre-emption with on-line scheduling policies only. 
% With off-line scheduling strategy, preemption is not allowed, but this limitation can be leveraged on the off-line scheduler side and a modification of the task version implementation, e.g. splitting the preempted task in two different tasks scheduled consecutively to the pre-emptor.
% Pre-emptions arise after the on-line scheduler sorted the ready queue.
%, either the worker ready queue or the global ready queue depending on the scheduling strategy. 
Upon sorting, similarly to \cite{mollison2013bringing}, the scheduler thread sends a signal (PREEMPTION\_SIGNAL), using the \textit{pthread\_kill} POSIX primitive, to each worker thread executing tasks with a lower priority than the head of the ready queue. This signal is caught by the thread which looks in the ready task queue for a higher priority task at the head of the ready queue. If a higher priority task is found, the execution context of the pre-emptee is saved (task with lower priority), and a context switch to the pre-emptor is operated (task with a higher priority). Upon the pre-emptor completion, the process of finding a higher priority task is repeated until the pre-emptee becomes the highest priority task, and the context is switched back to this task. 

\textbf{Locking: }
Internally, we implemented synchronisation primitives, i.e. mutexes or barriers, in two different manners. A first implementation uses the POSIX API implemented in the kernel and GLibC. A second implementation relies on lock-free algorithm from \cite{mellor1991algorithms}. It is possible to select one of the two options at compile time using the configuration file. We believe that lock-free algorithms is a better option for users wishing to perform a static WCET analysis, but spinlocks exhibit a higher energy consumption. On the other hand, it is hard to analyse kernel and GLibC calls, but it offers better energy performance at the cost of predictability due to the kernel replacing the worker thread by internal idle task. Selecting one or the other depends on user desired thresholds between predictability and energy conservation.

\textbf{Scheduling hooks: }
All end-user RT tasks are internally wrapped. This wrapping task allows us to call pre-scheduled and post-scheduled hooks defined by the user. Hooks can be useful to, for example, detect faulty behaviour by observing and profiling the miss-cache ratio of a task. Upon detection of an error, the hook can advise our scheduler to use a different version of the current task. Using a wrapping task allows us to keep this behaviour outside of the end-user code, which can focus only on the code of the feature, and allows us to keep this behaviour whether we are on a normal task execution or in a preemption state.

\textbf{Protecting against page fault: }
Similarly to \cite{mollison2013bringing}, we lock our library code in memory using the POSIX primitive \textit{mlockall}. This prevents swapping out the code of our library.

\textbf{Context switching: }
Similarly to \cite{mollison2013bringing}, we implemented a architecture dependent \textit{swapcontext} function (in assembly code), which is called when switching execution context upon pre-emption. %It therefore brings us the same benefits and drawbacks as them.
We draw inspiration from the GLibC swapcontext implementation, but removed extra syscalls. As of writing it is available for ARM 32/64 bits, as well as X86-64 architectures.
%We benefit from a fast context switch which has no extra syscall, as found in GLibC swapcontext implementation. And 
%The drawback lies in architecture support as this function is implemented in assembly code.

\textbf{Interrupts: }
Software interrupt handler mappings can be configured at the kernel level. We therefore configure the kernel to use the dedicated core that will neither run a worker thread, nor run the scheduler thread. %This can be achieve ...

We set the kernel to use \textit{threadirq}, and we shield the processor using \textit{isolcpu}. Hardware interrupt handlers are composed of two parts, a top and a bottom half. We cannot do much about the top half that usually is pinned to a specific core. For the bottom half, if they are not pinned to a specific core, then the same configuration as for software interrupts applies. If they are specific to a core, and this core runs a worker thread, or the scheduler thread, then their schedule is left to the underlying OS. Care must therefore be taken to ensure that the priority of our worker threads, and/or scheduler threads allows these bottom half interrupt handlers to execute.

% \paragraph{Other Linux specific configuration}

% Other levers can be pulled to increasing the timing control over a Linux-based kernel. Some of them are detailed in \cite{rouxel2020prego}.

\textbf{Standard compliance: }
We engineered our library to facilitate its analysis by standard WCET tools as much as possible.
Nonetheless, our library is a middleware that acts in between the kernel and end-user application, forcing us to the kernel API with syscalls. But most of the syscalls are performed outside of the \textit{\APIprefix start} and \textit{\APIprefix stop}, hence not interfering with the real-time end-user tasks. In addition, we provide the possibility to use either lock-free implementation of the FIFO mutex semaphores, or the POSIX mutex primitives. Thus, our library can be used in a deployed environment as much as prototyping a real-time system.

% Except few exceptions, we rely on POSIX standard API, thus enabling easy portage of our library to many OSes as well as targetted platforms. In addition, most of the time-wise hazarding POSIX primitive calls are performed when initialising or exiting the application, thus interfering as few as possible with the rt tasks and scheduling process.

% \subsection{Configuration}

% To avoid dynamic allocation, and customise our middleware to the end-user desires (in terms of scheduling policy), we use a C header configuration file. This header file embeds a series of pre-processor definitions that will activate or deactivate some parts of the library, initialise statically allocated structures and so one. Table \ref{tbl:coord:conf} presents the pre-processor constants to define in this configuration file.

% \begin{sidewaystable}[h!t]
% 	\caption{\label{tbl:coord:conf}Configuration possibilities}
% 	\begin{tabular}{|l|l|}
% 		\hline
% 		Parameter & Comment\\
% 		\hline
% 		\APIprefix MGNT\_MAIN\_THREAD\_AFFINITY & CPU id to map the main thread \\
% 		\APIprefix MGNT\_ALARM\_CLOCK & Clock id for the on-line scheduler (e.g CLOCK\_MONOTONIC)\\
% 		\APIprefix MGNT\_NB\_PERIODIC\_TASKS & Number of periodic tasks\\
% 		\APIprefix THREAD\_POOL\_NB\_THREADS & Number of threads\\
% % 		\APIprefix THREAD\_POOL\_THREAD\_NAME & A general name for the thread\\
%         \APIprefix THREAD\_POOL\_PREEMPTION\_MODEL & Preemption model to use\\
%         & \APIprefix PREEMPTIVE\\
%         & \APIprefix NONPREEMPTIVE\\
% 		\APIprefix THREAD\_POOL\_AFFINITIES & Thread-core mapping, e.g. {4,5,6} places the 3 created threads on respectively core id 4,5, and 6.\\
% 		\APIprefix THREAD\_POOL\_PRIORITIES & Thread system priority, e.g. {10,15,42} sets respectively priority 10,15, and 42 to the 3 created threads \\
% 		\APIprefix THREAD\_MAPPING & Mapping scheme to use for the user tasks, can be one of the 3: \\
% 		& \APIprefix THREAD\_MAPPING\_GLOBAL\_SCHEME\\
% 		& \APIprefix THREAD\_MAPPING\_PARTITIONED\_SCHEME\\
% 		& \APIprefix THREAD\_MAPPING\_STATIC\_SCHEME\\
% 		\APIprefix THREAD\_PRIORITY\_ASSIGNMENT & Priority assignment scheme for the user's tasks, can be on of \\
% 		& \APIprefix TASK\_PRIORITY\_RM\\
% 		& \APIprefix TASK\_PRIORITY\_DM\\
% 		& \APIprefix TASK\_PRIORITY\_FIFO\\
% 		& \APIprefix TASK\_PRIORITY\_USERPRIO\\
% 		\APIprefix TASK\_POOL\_NB\_TASKS & Maximum number of tasks including the periodic ones\\
% 		\APIprefix TASK\_NB\_VERSION\_MAX & Maximum number of variants\\
% 		\APIprefix SYNCHRO\_FORCE\_POSIX & To force using POSIX synchronisation primitives instead of lock-free algo\\
% 		\APIprefix HOOK\_PRE\_TASK\_CALL & Hook function to call before executing any task pre\_task\_hook\_func\\
% 		\APIprefix HOOK\_POST\_TASK\_CALL & Hook function to call after executing any task post\_task\_hook\_func\\
% 		\hline
% 	\end{tabular}
% \end{sidewaystable}

% \subsection{A generative approach}

% To facilitate the use of our library, we also develop a tool that from a high level description of the application will generate both the configuration file to use our library as well as the main C code file. We describe the high level DSL language that we created to describe an application in \cite{roeder2020towards}, and reported a use-case study following the generative approach in \cite{rouxel2020prego}.

==> sections/overhead.tex <==
\section{\label{sec:overhead}Overhead and Latencies}

%The implementation details from Section~\ref{sec:implem} identified the overhead location hereafter described in more depth. 

Scheduling overhead only occurs at schedule time. the time required to initialise or close the library is left aside as not interfering with the end-user RT tasks. The theoretical time $0$ present in the scheduling theory is considered to be time of the first invocation of the scheduler.

% Due to the design constraints of our library, we have few overheads. Indeed, it is not possible to alter the task set (adding/removing) while the schedule is running, see Sec \ref{sec:implem:gen}. Therefore, we note three types of overhead having an impact on the task WCET and latencies. All other overhead and latencies, including among other: thread spawning and joining, can be left aside as they never arises when executing the critical part of the application.


% \paragraph{Starting \& Stopping the schedule}

% This additional latency arises between the API call to \textit{coord\_start} and the actual execution of the first tasks at the theoretical time $0$. Respectively when stopping the schedule, there is an additional latency between the API call to \textit{coord\_stop} and the actual completion of currently executing tasks.

\subsection{Identified overheads}

\paragraph{Get task time}
The get-task overhead is present only for on-line scheduling policies, as there is no shared ready queue for the off-line dispatcher. 

In case of partitioned scheduling, a worker thread does not have to wait for other threads to release the ready queue as the ready queue is on a per-thread basis. 
Due to the FIFO, each worker thread can be blocked only $1*Scheduling~ Time$. On the other hand, the scheduler thread can be blocked for $N$ \textit{Get Task Time} by other thread.
% Therefore, the \textit{Get Task Time} is equal to the \textit{Scheduling Time}.

On the other hand with global scheduling, to get a task from the ready queue, a worker thread requests access to the mutually exclusive shared resource through a FIFO mutex semaphore. Once access is granted, the worker thread removes the task from the head and releases the lock. 
%The size of the critical section is very small (about .. assembly lines). 
This critical section is executed by all worker threads, and a worker thread can be blocked by $(N-1)$ threads, so $(N-1)\times Get~Task~Time$, and $1 * Scheduling~ Time$.
%In addition, the scheduler thread might want to access the ready queue for $1 * Scheduling~ Time$.
Similarly, the scheduler thread can be blocked for $N*Get~Task~Time$ by other thread.

\paragraph{Scheduling time}

Similarly to the get-task overhead, the scheduling-time overhead applies only to on-line schedulers. The scheduler locks the ready queue, then scans the task list to decide which one has reached its arrival time. If a task needs to be released, then it is placed in the ready queue. Upon scanning the list of tasks, the ready queue is sorted, and the lock is released. The size of the critical section is dependent on the number of tasks which is \textit{a priori} known. In the worst-case, the critical section corresponds to add all tasks in the ready queue plus a sorting the queue.

% With global scheduling policy, and due to the FIFO mutex semaphore, thread interrupt handlers can be blocked by $(N-1)*get~task~time$.

\subsection{A Global Overview of overheads}

\paragraph{Task management}

The task-management overhead must be added to each task's WCET. It corresponds to the time interval between the theoretical release time of a task and its effective release time, and the time interval between its theoretical completion and its effective completion. Figure \ref{fig:overhead:reg-task} details the overhead added before and after the isolated WCET of a task for on-line and off-line schedulers. Between the two scheduler types, only the hatched part differs and is not present when dealing with off-line schedulers.

% in Figure \ref{fig:overhead:reg-task:on-line}, and off-line schedulers in Figure \ref{fig:overhead:reg-task:off-line}.

\begin{figure}[ht]
    % \begin{subfigure}{0.5\textwidth}
	    \centering
        \includegraphics[scale=0.4]{figures/OverheadReleaseTask.pdf}
		\caption{Effective task execution time with overhead. The hashed part is present only for on-line schedulers.}
		\label{fig:overhead:reg-task}
% 	\end{subfigure}

% 	\begin{subfigure}{0.5\textwidth}
% 	    \centering
%         \includegraphics[scale=0.4]{figures/OverheadOffLine.pdf}
% 		\caption{Effective task execution time for off-line schedulers}
% 		\label{fig:overhead:reg-task:off-line}
% 	\end{subfigure}

% 	\caption{Effective task WCET with additional overhead details.}
% 	\label{fig:overhead:reg-task}
\end{figure}

\paragraph{Pre-emption management}

% We identified two overhead cases when dealing with pre-emption, one considers the pre-emptor (the higher priority pre-empting task), and the pre-emptee (the lower priority pre-empted task).
% Figure \ref{fig:overhead:pre-emptor} completes prior Figure \ref{fig:overhead:reg-task} by exhibiting the additional overhead on the pre-emptor, while Figure \ref{fig:overhead:pre-emptee} pictures a scenario on a pre-emptee.

Figure \ref{fig:overhead:pre-emption} displays the related overhead to a low priority task pre-empted by a higher priority one.

\begin{figure}[ht]
% 	\begin{subfigure}{0.5\textwidth}
	    \centering
	    \includegraphics[scale=0.4]{figures/OverheadPreemption.pdf}
% 		\caption{Additional overhead arising on a pre-emptor}
% 		\label{fig:overhead:pre-emptor}
% 	\end{subfigure}

% 	\begin{subfigure}{0.5\textwidth}
% 	    \centering
% 	    \includegraphics[scale=0.4]{figures/OverheadPreemptee.pdf}
% 		\caption{Additional overhead arising on a pre-emptee}
% 		\label{fig:overhead:pre-emptee}
% 	\end{subfigure}

	\caption{Effective task WCET with additional \textit{pre-emption} overhead details.}
	\label{fig:overhead:pre-emption}
\end{figure}



==> sections/rebuttal.tex <==
We thank all the reviewers for their insightful remarks that will help us to improve our manuscript. To clarify what we believe to be a misunderstanding, the idea behind YASMIN is to support more scheduling algorithms on heterogeneous COTS HW/OS, thus systems that are usually exotics and where a proper RTOS or LITMUS can't run. Following are the answers to the reviewers' questions.

\paragraph{To reviewer 1}~\\~ 
* We agree that the use case provided by our industrial partner is not adequate to demonstrate the full range of benefits of YASMIN. Unfortunately, there is a typo in the text: it is not 1s per image, but 10s per image in average that the CNN requires. From our experiments YASMIN does scale well with the number of tasks, but the user code does not scale up to larger installation sizes, and this problem is orthogonal to YASMIN. 
* Let's say you have 2 independent tasks where both have a CPU and a GPU version. Let's assume they have periods which will lead to have them running in parallel at some point in time. On the architecture there is only one GPU available. Therefore only one task can access the GPU, leaving the other one to wait for the shared resource. Having both implementations available at runtime allows to run the CPU version of the latter task while the GPU is busy with the former. A second scenario would lie in execution modes: a low energy execution mode would prefer the CPU versions, while a faster but more energy consuming would use the GPU.

\paragraph{To reviewer 2}~\\~
* We would require further experiments to validate this, but my educated guess is as follows: Remaining on a single cluster, e.g. the big cores, will speed up the scheduling process of YASMIN (as big cores are faster), at the detriment of losing a core for users' tasks (a core is reserved for the scheduling). YASMIN overheads will then be lower.
* LITMUS is not a middleware but rather a full kernel. It is a modified Linux. In that sense we propose a middleware that runs atop a kernel/OS. LITMUS can't be executed on exotic hardware, whereas our middleware can, as long as a POSIX OS can be executed on the HW.

\paragraph{To reviewer 3}~\\~
* Our middleware can be executed on any POSIX-compliant system at the exception that we need the non-POSIX function \textit{pthread\_set\_affinity\_np} to map threads on cores. If the OS is non-RT, there are many levers to pull to increase control over timing. Unfortunately, we can't give you the reference due to the double-blind restriction (bib reference [8] is hidden). 
* Our middleware can be used for scheduling exploration. A killer app would be any application running on exotic heterogeneous systems.
* (point 5) Switching is done at compile time, not at runtime. There is no induced switching overheads as only one scheduling policy remains after compilation. The compiled scheduling policy depends on some users' configuration given as C macros in a header file. This will configure the library and required parameters to provide when adding a task.

\paragraph{To reviewer 4}~\\~
* The memory hierarchy interference study is left for future work. A first hint would be to employ cache partitioning.
* We do not wish to extend the OS as in previous works as it would make our work dependent on OS versions, hence less maintainable.
* SCHED\_DEADLINE is not always available, e.g. it is not in the Linux version provided for the TK1. LITMUS can't run on all platforms, or embrace the heterogeneity, e.g. we are not aware of the possibility to use CUDA drivers.


==> sections/use-case.tex <==
\section{\label{sec:use-case}Parking Lot Monitoring Use-Case}

An industrial partner provided us with a use-case involving Convolutional Neural Networks (CNNs) performing object detection on images. The goal of the use-case is to monitor available parking lots (in a parking space) and determines if a car is parked in a lot or if the lot is free. %It can be used either autonomously or as part of a greater smart car-parking system in larger scale. 
Combining real-time requirements, rapid prototyping, scheduling exploration and task implementation exploration are the leitmotiv brought by our industrial use-case (described in Section \ref{sec:use-case}) for the creation of our middleware. 
As compared to previous approaches \cite{mollison2013bringing, saranya2014implementation}, \LibName~ enables various scheduling policies, task models and platforms with a simple API.

A tiny camera is placed above each parking spot, and each camera takes a picture every 30 seconds. The picture is then stored on a shared central hard drive disk with a name embedding the spot number and a timestamp. An Apalis TK1 from Toradex \cite{toradextk1} loads the images, executes a CNN trained to detect the presence of the car. The outcome of the CNN is then gathered and a message is send to a central unit to display the  available spots  and further statistics. Finally the picture is deleted. Our focus is only on the TK1 part, and we ignore the constant latencies to transfer pictures from cameras to the storage  and the time to send the result. Nonetheless to avoid loss of images, and display a meaningful information regarding the number of available spots, images ballot must be treated during the period (implicit deadline) before the next one arrives.

CNNs are computationally demanding mathematical structures, involving convolution operations between large 3D matrices (tensors) or multiplication of matrices of large dimensions. Use-cases relying on a deep-learning system, require a relatively strong computing system. 
%In the scope of TeamPlay, Irida Labs
The use-case provider
selected the Apalis TK1 from Toradex, as it meets all the performance criteria and a 10 years life support. This TK1 SoC provides an ARM Cortex-A15 CPU, 2 GBytes of DDR3 RAM memory, 16 GB of non-volatile eMMC storage, and an NVIDIA Kepler GPU with 192 CUDA cores. The platform is shipped with Ubuntu/Linux v3.10.40 and no PREEMPT\_RT patch set is available due to vendor specific drivers.

%tend to choose an ARM-based heterogeneous multi-core platform such as the ARM Cortex-A15. Besides general-purpose processors (CPUs) and specialized co-processors, the availability of a GPU is always a plus, given its suitability to execution of algorithms with the same nature as the CNN ones. The existence of a GPU decisively eases the implementation and execution of deep-learning algorithms, extending the available options for a heterogeneous programming scheme. Such a system could support applications in markets as diverse as Mobile Devices, Automotive and Industrial Inspection/Automation. 
% Making use of one of such platforms could lead to the implementation of a deep-learning system able to operate in real-time. 

The number of spots available in the parking is not a priori known as it depends on the actual deployment location of the system. Our industrial partner wishes to explore the possibility regarding the schedule of the application with a varying number of parking spots, thus determining a bound of usability. To utilise at most the TK1 platform, they also would like to determine the number of images that can be concurrently processed.
A schedulability analysis would be sufficient to answer these questions. However, it is hardly doable on such complex platform.

% Systems like that could find applications in Markets such as Mobile Devices, Automotive Industrial Inspection/Automation, IoT, space sector etc., for carrying-out tasks related to recognition of images, signals, etc. Depending on the application, the type and capacity of the required processing resources can vary significantly. 


\begin{figure}[ht]
    \begin{subfigure}{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Irida_Example-20-Input-Images.png}
        \caption{Example of input images}
        \label{fig:uc:ex}
    \end{subfigure}
    
    \begin{subfigure}{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/IridaSDF.pdf}
        \caption{SDF graph of the use-case}
        \label{fig:uc:graph}
    \end{subfigure}
    \caption{Use-case overview}
\end{figure}

The application includes a set of tasks implemented using C++ source code. 
The CNN that resides in the core of this system consists of 4-D convolution layers, MaxPool layers and a final FC layer with two nodes, corresponding to two target classes: either the lot is occupied or not. Some example images that the CNN model could be called to classify are shown in Figure \ref{fig:uc:ex}. The model has been trained off-line on a custom database of 74000 training images and 1306 validation images.

Tasks are organised following the Synchronous Dataflow Graph (SDF) from Figure~\ref{fig:uc:graph}. The graph includes 5 tasks. Labels on edges of the figure expressed the quantity of data exchanged between the tasks. As enabled by SDF graphs, the production of the source node and its direct successor do not match, thus requiring an expansion of the graph before scheduling and executing the application. 

We experimented the use of \LibName~ on this use case. We used the various set of scheduling policies presented in Section \ref{sec:exp} with the addition of preemptive and non-preemptive policies. To fill \LibName~ requirements we use two cores for worker threads, one core for the scheduler thread, leaving one core for the system. We varied the number of parking lot in $[1;5]$ with a step of $1$, and left the application run for 10 periods (1 period = 30seconds / number of parking lots). Even if it is difficult to demonstrate it here, we want to stress how easy it was to prepare these 240 \footnote{$5 parking config * 8 scheduling policies$} test cases by just minor modifications of the configuration file. Indeed, relying on \LibName~ helps to focus only on the body of the tasks, leaving the middleware do all the synchronisation.

% \begin{figure}[ht]
%     \centering
%     % \includegraphics[width=0.5\textwidth]{figures/use-case-stats.png}
%     \includegraphics[width=0.5\textwidth]{figures/use-case-stats-deadline.png}
%     \caption{Processing time per image depending on the number of parking slot}
%     \label{fig:uc:time}
% \end{figure}
% Figure \ref{fig:uc:time} presents the number of deadline misses per scheduling policies.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/use-case-stats.png}
    \caption{Processing time per image depending on the number of parking slot}
    \label{fig:uc:time}
\end{figure}

Figure \ref{fig:uc:time} presents our measurements for the various preemptive (P) and non-preemptive (NP) scheduling policies running on the TK1. 
%Except few outliers the processing time per frame remains steady, leaving several possibilities for the choice of the scheduling policy.
Using \LibName, we were able to identify the optimal number for scheduling for a given number of parking spots. Even though the system does not scale to large parking areas mostly due to the execution time of the CNN (about 1 second per image), this experiment shows the applicability of our library on industrial application, and that picking the right scheduling policy is not trivial.

